Towards an Asset Administration Shell Maturity Model

The Asset Administration Shell (AAS) is increasingly recognized as a fundamental model for the realization of and data exchange between digital twins in manufacturing. An AAS defines a hierarchical data structure to represent any type of asset throughout its entire lifecycle. In the context of AAS-based systems, comparing different AAS instances constitutes a practical challenge, as neither a widely accepted methodological framework nor a maturity model are available to systematically support such analyses. To address this gap, we propose a novel concept of AAS maturity that characterizes the extent to which established digital twin criteria are met and thus enabling comparability of AAS instances. The concepts are derived from the literature and applied through exemplification. These emerging results enable practitioners and researchers to systematically compare AAS instances and support the identification and assessment of further development steps in the digital twin engineering process.

==> Figures/spider-plot-fivex.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[font=\LARGE]

% ---- Parameter ----
\def\max{6} % Maximum radius (Services has 6 levels)

% ---- Colors for data points ----
\definecolor{c1}{RGB}{31,119,180}
\definecolor{c2}{RGB}{255,127,14}
\definecolor{c3}{RGB}{44,160,44}
\definecolor{c4}{RGB}{214,39,40}
\definecolor{c5}{RGB}{148,103,189}

% ---- Axes Angles ----
\def\aA{90}
\def\aB{18}
\def\aC{-54}
\def\aD{-126}
\def\aE{-198}

% ---- Spider grid (grey) ----
\foreach \r in {2,...,6}{
    \draw[gray!50] (0,0) \foreach \a in {\aA,\aB,\aC,\aD,\aE, \aA}
        {-- (\a:\r)} -- cycle;
}

% Axes
\foreach \a in {\aA,\aB,\aC,\aD,\aE}
    \draw[gray!70] (0,0) -- (\a:\max);

% ---- Axis Labels ----
\node at (\aA+2:\max+0.8) {\textbf{Connection}};
\node at (\aB-3:\max+0.8) {\textbf{Data}};
\node at (\aC:\max+0.8) {\textbf{Services}};
\node at (\aD:\max+0.8) {\textbf{Physical Entity}};
\node at (\aE:\max+0.8) {\textbf{Models}};

% ---- Data Points ----
% Connection (3)
\fill[c1] (\aA:2) circle (2pt) node[right=2pt, rotate=36] {Manual Data Flow};
\fill[c1] (\aA:4) circle (2pt) node[right=2pt, rotate=36] {Unidirectional Automated Data Flow};
\fill[c1] (\aA:6) circle (2pt) node[right=2pt, rotate=36] {Automated Data Flow};

% Data (3)
\fill[c2] (\aB:2) circle (2pt) node[right=2pt, rotate=36] {No Synchronization};
\fill[c2] (\aB:4) circle (2pt) node[right=2pt, rotate=36] {Parial Synchronization};
\fill[c2] (\aB:6) circle (2pt) node[right=2pt, rotate=36] {Synchronization};

% Services (6)
%\fill[c3] (\aC:1) circle (2pt) node[right=2pt] {1 out of 6 Service Categories Included};
\fill[c3] (\aC:2) circle (2pt) node[right=2pt, rotate=36] {No Services Included};
%\fill[c3] (\aC:3) circle (2pt) node[right=2pt] {3 out of 6 Service Categories Included};
\fill[c3] (\aC:4) circle (2pt) node[right=2pt, rotate=36] {Services from 3 Different Categories Included};
%\fill[c3] (\aC:5) circle (2pt) node[right=2pt] {5 out of 6 Service Categories Included};
\fill[c3] (\aC:6) circle (2pt) node[right=2pt, rotate=36] {Services of All Categories Included};

% Physical Entity (3)
\fill[c4] (\aD:2) circle (2pt) node[right=2pt, rotate=36] {Intangible Asset };
\fill[c4] (\aD:4) circle (2pt) node[right=2pt, rotate=36] {Physical Asset Planned};
\fill[c4] (\aD:6) circle (2pt) node[right=2pt, rotate=34] {Physical Asset Implemented};

% Models (3)
\fill[c5] (\aE:2) circle (2pt) node[right=2pt, rotate=36] {Empty Models};
\fill[c5] (\aE:4) circle (2pt) node[right=2pt, rotate=36] {Semi-complete Models};
\fill[c5] (\aE:6) circle (2pt) node[right=2pt, rotate=36] {Complete Models};

% ---- Filled Data Polygon ----
\draw[color=black!80, fill=red!40, fill opacity=0.2] 
    (\aA:2) -- 
    (\aB:3) -- 
    (\aC:2) -- 
    (\aD:4) -- 
    (\aE:2.5) -- cycle;

\draw[color=black!80, fill=green!40, fill opacity=0.2] 
    (\aA:2) -- 
    (\aB:4.3) -- 
    (\aC:3.5) -- 
    (\aD:4) -- 
    (\aE:4.8) -- cycle;

\draw[color=black!80, fill=blue!40, fill opacity=0.2] 
    (\aA:5.2) -- 
    (\aB:5) -- 
    (\aC:4.5) -- 
    (\aD:6) -- 
    (\aE:5.4) -- cycle;
    

% ---- Legend ----
% \begin{scope}[shift={(9,-4)}]
% \node[anchor=west] at (0,4.5) {\textbf{Legend}};
% \foreach \txt/\col/\y in {
% C1/c1/4.2, C2/c1/3.9, C3/c1/3.6,
% D1/c2/3.3, D2/c2/3.0, D3/c2/2.7,
% S1/c3/2.4, S2/c3/2.1, S3/c3/1.8,
% S4/c3/1.5, S5/c3/1.2, S6/c3/0.9,
% P1/c4/0.6, P2/c4/0.3, P3/c4/0.0,
% M1/c5/-0.3, M2/c5/-0.6, M3/c5/-0.9}
% {
% \fill[\col] (0,\y) circle (2pt);
% \node[anchor=west] at (0.3,\y) {\txt};
% }
% \end{scope}
\begin{scope}[shift={(4,4)}]
\node[anchor=west] at (0,1.5) {\textbf{Legend}};
\fill[red!40] (0,1.1) circle (2pt);
\node[anchor=west] at (0.3,1.1) {Early AAS};
\fill[green!40] (0,0.7) circle (2pt);
\node[anchor=west] at (0.3,0.7) {Developed AAS};
\fill[blue!40] (0,0.3) circle (2pt);
\node[anchor=west] at (0.3,0.3) {Integrated AAS};


\end{scope}

\end{tikzpicture}
}
